MOS-Bias: From Hidden Gender Bias to Gender-Aware Speech Quality Assessment

The Mean Opinion Score (MOS) serves as the standard metric for speech quality assessment, yet biases in human annotations remain underexplored. We conduct the first systematic analysis of gender bias in MOS, revealing that male listeners consistently assign higher scores than female listeners--a gap that is most pronounced in low-quality speech and gradually diminishes as quality improves. This quality-dependent structure proves difficult to eliminate through simple calibration. We further demonstrate that automated MOS models trained on aggregated labels exhibit predictions skewed toward male standards of perception. To address this, we propose a gender-aware model that learns gender-specific scoring patterns through abstracting binary group embeddings, thereby improving overall and gender-specific prediction accuracy. This study establishes that gender bias in MOS constitutes a systematic, learnable pattern demanding attention in equitable speech evaluation.

==> Tables/BVCC_listener_numbers_with_gender.tex <==
\begin{table}[t]
\centering
\caption{Average number of male and female listeners per sample across BVCC data splits.}
\label{tab:BVCC_listener_numbers_with_gender}
\begin{tabular}{lcc}
\toprule
\textbf{Split} & \makecell{\textbf{Avg. Number of}\\\textbf{Male Listeners}} & \makecell{\textbf{Avg. Number of}\\\textbf{Female Listeners}} \\
\midrule
Train & 3.66 & 4.25 \\
Dev   & 4.05 & 3.72 \\
Test  & 3.58 & 4.33 \\
\bottomrule
\end{tabular}
\end{table}

==> Tables/SHEET_Datasets_Gender_Metadat.tex <==
\setlength{\tabcolsep}{4pt}
\begin{table}[t]
\centering
\caption{Availability of speaker/listener labels and gender metadata across MOS-Bench training datasets. Only BVCC provides gender annotations for both speakers and listeners.}
\label{tab:sheet_gender_metadata}
\begin{tabular}{lcccc}
\toprule
\raisebox{-0.5\normalbaselineskip}{\textbf{Dataset}} & \makecell{\textbf{Speaker}\\\textbf{Label}} & \makecell{\textbf{Listener}\\\textbf{Label}} & \multicolumn{2}{c}{\textbf{Gender Annotation}} \\
\cmidrule(lr){4-5}
 & & & Speaker & Listener \\
\midrule
BVCC       & \cmark & \cmark & \cmark & \cmark \\
SOMOS      & \omark  & \cmark & \xmark  & \xmark  \\
SingMOS    & \xmark  & \xmark & \xmark  & \xmark  \\
NISQA      & \cmark & \xmark  & \xmark  & \xmark  \\
TMHINT-QI  & \cmark & \cmark & \cmark & \xmark  \\
Tencent    & \cmark & \xmark  & \xmark  & \xmark  \\
PSTN       & \cmark & \xmark  & \xmark  & \xmark  \\
\bottomrule
\end{tabular}

\vspace{2pt}
\footnotesize
\noindent
SOMOS(\omark) uses a single speaker, \textit{Speaker/Listener Label} indicates whether individual speaker/listener identifiers are provided. \textit{Gender Annotation} indicates the availability of gender metadata for speakers and/or listeners.
\end{table}
